Cloud, Fog or Edge: Where to Compute?

The computing continuum extends the high-performance cloud data centers with energy-efficient and low-latency devices close to the data sources located at the edge of the network. However, the heterogeneity of the computing continuum raises multiple challenges related to application management. These include where to offload an application - from the cloud to the edge - to meet its computation and communication requirements. To support these decisions, we provide in this article a detailed performance and carbon footprint analysis of a selection of use case applications with complementary resource requirements across the computing continuum over a real-life evaluation testbed.

==> old.tex <==


We use TensorFlow as the most popular ML library, which provides a collection of workflows to develop and train models using different programming languages.

The industry primarily uses TensorFlow due to the wide community support and easy portability. TensorFlow supports different heterogeneous computing architectures (x86-64, ARM, specialized processors, TPUs and GPUs) and operating systems (Windows, Linux, Pi OS, MacOS), which makes it suitable for the deployment across the computing continuum.

Multiple essential IoT applications, such as smart cities and connected health care rely on in-memory data analytic to provide services. We therefore explore data analysis from a perspective of inspecting, filtering and transforming of data for exposing useful knowledge and aiding the decision-making process. 

For the data analytic purpose, we identify \textit{Apache Spark}\footnote{https://spark.apache.org} as the most representative engine

for distributed large-scale in-memory data processing and analytic, which encompasses stream processing, machine learning, interactive analytic and data integration. It supports different programming languages on top of Hadoop, Kubernetes or standalone cloud instances, fog and edge devices. This makes it suitable for processing big data on the computing continuum. 



In addition, Exoscale provides a dedicated 32-core server, located at the 5G Playground in Klagenfurt and available on demand through the Exoscale API.


Video encoding allows transmission of video content with different qualities over limited and heterogeneous communication channels, such as the Internet. It is the process of compressing an original raw video to reduce its bandwidth consumption, while maintaining the subjective quality for viewers as high as possible.


ML is a branch of artificial intelligence that explores approaches for enabling systems to learn from data, identify patterns and make decisions with minimal human intervention. Its applications include autonomous vehicles, recommender systems and natural language understanding, among others.

%In relation to the in-memory analysis in Spark we furthermore perform evaluation on the memory performance by measuring time required to load the input data from the local SSD storage into the main memory for the collaborative filtering scenario. We depict the results in Figure~\ref{fig:mem}. Here it can be observed that all \texttt{x86}-based devices show better performance than the \texttt{ARM} devices. This is due to the more complex memory controller and memory modules utilized in the enterprise-level hardware. 
%\input{Figures/memory}

%\section{CONCLUSION}
%In this article we present a performance and environmental analysis of devices and instances across the computing continuum, intended to aid the decision process when to offload to the edge of the network. Therefore, we have utilized a representative set of applications, which cover a broad set of use cases essential to the industry and academia. 
%here Dragi to add stronger reasons. 
%Our analysis highlights the recent advances in microprocessor design, which enable creation of small and energy-efficient devices with high computational performances, such the Raspberry Pi4 and Jetson Nano, to be deployed closer to the data sources. We can further conclude that the current edge and fog devices, based on arm architectures, can provide performance similar to the cloud, especially in situations when the resource utilization is lower. On the other hand, when multiple applications have to share the same hardware or need scalability, in terms of computing resources, then the cloud remains the optimal platform of choice.   
%Lastly from the environmental point of view, it is clear that partial offloading of distributed IoT applications to the fog and edge can reduce significantly the carbon footprint and contribute towards reducing the global warming. 
%\section{ACKNOWLEDGMENT}


%The testbed has a fiber-optic connection to the Exoscale cloud with a maximum bandwidth of \SI{10}{\giga\bit\per\second}. 

%Finally, our analysis also highlighted the recent advances in microprocessor design, which enable creation of small and energy-efficient devices with high computational performances, such the Raspberry Pi4 and Jetson Nano, to be deployed. We can further conclude that the current edge and fog devices, based on \texttt{arm} architecture, can provide slightly worse performance compared to the cloud, but only in situations when the resource utilization is lower. On the other hand, when scalability of resources is essential the cloud remains the optimal platform of choice.



% I THINK THIS SECTION IS NOW NOT NEEDED, AS WE HAVE RECOMMENDATIONS AFTER EACH APPLICATION. SO I REMOVED IT. 

%\section{Considerations for IoT application offloading}
%Subsequently, based on the performance evaluation and carbon emission characterization, we derive a short guide for practitioners that should be considered when offloading an IoT application: 



%\begin{itemize}
%    \item Characterize the IoT application in terms of core algorithms as described in Table \ref{tbl:use-case}; 
   % \item Identify the interactions among the components of the IoT applications, in terms of frequency and size of data transfers;
%    \item Identify the core algorithms utilized by the IoT application, such as video encoding, machine learning or filtering;
   % \item Perform preliminary measurement on the execution time and data transfers on a small set of available resources with similar characteristics like the ones presented in this article;
%    \item Utilize the results from the performance evaluation over the $C^3$ testbed to estimate the execution and data transfer times across various devices and instances you may want to use;
%    \item Utilize the results from our environmental analysis to estimate the carbon emissions;
    %\item If the IoT application has tight latency requirements with high frequency of small sized data transfers (i.e. live video) use the performance evaluation to identify, which cloud, fog or edge device could satisfy the requirements and offload there;
%    \item If the IoT application is not time sensitive and the data transfers is constant (i.e., video on demand) offload to the fog and edge; 


%Fog and edge computing have a large potential to steer the extension of the cloud services to the sources of data.

%Consequently, the lack of direct characterization of the resources across the cloud, fog and edge hinders the transparent management of applications. 

%, intended to aid the decision process of where to offload an application, ranging from the cloud to the edge of the network. %For this purpose, we utilized a representative set of real-world applications, which cover a broad set of use cases essential to industry and academia. We utilized the gained insights to provide recommendations on where to offload different classes of applications, summarized in Table \ref{tbl:recomend}


%\begin{itemize}
%    \item The \emph{cloud layer} contains high-performance resources consolidated in vast data-centers.
%    \item The \emph{fog layer} comprises \highlight{public and private computing infrastructures consolidated in small data-centers} in the close vicinity to the data sources (i.e. within internet service provider network). 
%    \item The \emph{edge layer} encompasses commodity hardware, such as personal computers, smart mobile and Internet of Things (IoT) devices, located in the immediate vicinity of the data sources (i.e. within local area network).
%\end{itemize}


%\highlight{Our analysis gives recommendations to practitioners on where to deploy their applications in the cloud, fog and edge continuum.}

%\highlight{The time for transfer of the raw video segment from a storage device registered in the network of the Klagenfurt University to the respective device ranged from \SI{5.01}{\second} for the Raspberry Pi 4 and EGS to  \SI{170.1}{\second} for the AWS \texttt{c5.large} instance (see Figure \ref{fig:trans}).} 

%Nevertheless, for short video segments, the encoding time in Quad HD resolution took \SI{36}{\second} on average. 


\begin{table}[t]
\scriptsize
\caption{Complementary requirements overview of the selected application classes.}
\centering
{
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|}
\hline
 \backslashbox[23mm]{\textit{Application}}{\textit{Requirement}} &
 \textit{CPU} & \textit{Memory}& \textit{Effective throughput} & \textit{Latency} \\
\hline
\textit{Video encoding} &High & Low & High & Low/Medium  \\
\hline
\textit{Machine learning} & High & High & Low & Medium  \\
\hline
\textit{In-memory analytic} & Medium & High & Medium & Medium   \\
\hline
\end{tabular}
}}
\label{tbl:use-case}
\end{table}

\begin{table*}[t]
\caption{\color{dgreen}DeFog versus $C^3$ comparison.}
\centering
%{
%\resizebox{\textwidth}{!}{
\color{dgreen}
\begin{tabular}{|c|c|c|c|}
\hline
\backslashbox[23mm]{\textit{Aspect}}{\textit{Approach}} &
 \textit{DeFog} & \textit{$C^3$}  \\
\hline
\textit{Goal} & \makecell{Benchmark suite}  & \makecell{Offload recommendations}  \\
\hline
\textit{Application classes} & Individual services & \makecell{Complementary industrial applications\\ (encoding, machine learning, in-memory analytic)}\\
\hline
\textit{$CO_2$ analysis} & No & Yes \\
\hline
\textit{Continuum resources} & 1 cloud; 2 RPi 3B & \makecell{Larger $C^3$ testbed with 40 heterogeneous devices\\ (3 cloud, 4 fog, 1 EGS, 35 RPi 3B+ and 4B, 5 Jetson Nanos)}    \\
\hline
\textit{Performance analysis} & No (only metrics and evaluation) & \makecell{Detailed analysis with offload recommendations}    \\
\hline
\end{tabular}
%}}
\label{tab:defog}
\end{table*}


==> others.tex <==
\begin{figure}[h!]
    \centering
\begin{tikzpicture}[scale=0.6]
  \centering
  \begin{axis}[
        ybar, axis on top,
       % title={In-memory SPARK Performance Analysis},
        height=8cm, width=12cm,
        bar width=0.4cm,
        nodes near coords,
        every node near coord/.append style={rotate=90, anchor=west},
       % ymajorgrids, tick align=inside,
       major grid style={draw=black},
        enlarge y limits={value=.1,upper},
        ymin=0, ymax=6,
     %   axis x line*=bottom,
    %    axis y line*=right,
     %   y axis line style={opacity=0},
      %  tickwidth=0pt,
       % enlarge x limits=true,
        legend style={
            at={(0.5,-0.3)},
            anchor=north,
            legend columns=-1,
            font=\scriptsize,
            /tikz/every even column/.append style={column sep=0.5cm}
        },
        restrict y to domain*=0:117, % Cut values off at 14
    visualization depends on=rawy\as\rawy, % Save the unclipped values
    after end axis/.code={ % Draw line indicating break
            \draw [ultra thick, white, decoration={snake, amplitude=2pt}, decorate] (rel axis cs:0,1.01) -- (rel axis cs:1,1.01);
        },
        nodes near coords={%
            \pgfmathprintnumber{\rawy}% Print unclipped values
        },
        ylabel={Carbon emission (grams)},
        y label style = {xshift=-0.2em,font=\scriptsize},
         yticklabel style = {xshift=-0.2em,font=\scriptsize},
        symbolic x coords={
            RPi3,RPi3B, EdgeGW, EdgeS1vCPU, EdgeS2vCPU, EdgeS4vCPU, Cloudv1, Cloudv4, Cloudv8},
       xticklabel style = {rotate=45, xshift=-0.2em,font=\scriptsize},
       axis lines*=left,
         clip=false
    ]
    \addplot [color =blue, fill=blue!30] coordinates {
      (RPi3, 1.1)
      (RPi3B, 1.0) 
      (EdgeGW, 1.5)
      (EdgeS1vCPU, 2.3) 
      (EdgeS2vCPU, 4.1)
      (EdgeS4vCPU, 3.9) 
      (Cloudv1, 2.4)
      (Cloudv4,3.8) 
       (Cloudv8, 5.4)
       };
    \legend{Carbon emissions}
  \end{axis}
  
  \end{tikzpicture}
    \caption{Carbon footprint for training a neural network with accuracy of above 77\%}
    \label{fig:my_label}
\end{figure}

